Doubly Robust Monte Carlo Tree Search

We present Doubly Robust Monte Carlo Tree Search (DR-MCTS), a novel algorithm that integrates Doubly Robust (DR) off-policy estimation into Monte Carlo Tree Search (MCTS) to enhance sample efficiency and decision quality in complex environments. Our approach introduces a hybrid estimator that combines MCTS rollouts with DR estimation, offering theoretical guarantees of unbiasedness and variance reduction under specified conditions. Empirical evaluations in Tic-Tac-Toe and the partially observable VirtualHome environment demonstrate DR-MCTS's superior performance over standard MCTS. In Tic-Tac-Toe, DR-MCTS achieves an 88% win rate compared to a 10% win rate for standard MCTS. In compound VirtualHome tasks, DR-MCTS attains a 20.7% success rate versus 10.3% for standard MCTS. Our scaling analysis reveals that DR-MCTS exhibits better sample efficiency, notably outperforming standard MCTS with larger language models while using a smaller model. These results underscore DR-MCTS's potential for efficient decision-making in complex, real-world scenarios where sample efficiency is paramount.

==> Styles/reference.tex <==
@article{glass2013causal,
  title={Causal inference in public health},
  author={Glass, Thomas A and Goodman, Steven N and Hern{\'a}n, Miguel A and Samet, Jonathan M},
  journal={Annual review of public health},
  volume={34},
  pages={61--75},
  year={2013},
  publisher={Annual Reviews}
}

@article{athey2017estimating,
  title={Estimating heterogeneous treatment effects using machine learning},
  author={Athey, Susan and Imbens, Guido},
  journal={arXiv preprint arXiv:1510.04342},
  year={2017}
}

@book{imbens2015causal,
  title={Causal inference in statistics, social, and biomedical sciences},
  author={Imbens, Guido W and Rubin, Donald B},
  year={2015},
  publisher={Cambridge University Press}
}

@article{hill2011bayesian,
  title={Bayesian nonparametric modeling for causal inference},
  author={Hill, Jennifer L},
  journal={Journal of Computational and Graphical Statistics},
  volume={20},
  number={1},
  pages={217--240},
  year={2011},
  publisher={Taylor \& Francis}
}

@book{angrist2008mostly,
  title={Mostly harmless econometrics: An empiricist's companion},
  author={Angrist, Joshua D and Pischke, J{\"o}rn-Steffen},
  year={2008},
  publisher={Princeton university press}
}

@article{heckman2007econometric,
  title={Econometric evaluation of social programs, part I: Causal models, structural models and econometric policy evaluation},
  author={Heckman, James J and Vytlacil, Edward J},
  journal={Handbook of econometrics},
  volume={6},
  pages={4779--4874},
  year={2007},
  publisher={Elsevier}
}

@article{kang2007demystifying,
  title={Demystifying double robustness: A comparison of alternative strategies for estimating a population mean from incomplete data},
  author={Kang, Joseph DY and Schafer, Joseph L},
  journal={Statistical science},
  volume={22},
  number={4},
  pages={523--539},
  year={2007},
  publisher={Institute of Mathematical Statistics}
}

@article{funk2011doubly,
  title={Doubly robust estimation of causal effects},
  author={Funk, Michele Jonsson and Westreich, Daniel and Wiesen, Chris and St{\"u}rmer, Til and Brookhart, M Alan and Davidian, Marie},
  journal={American journal of epidemiology},
  volume={173},
  number={7},
  pages={761--767},
  year={2011},
  publisher={Oxford University Press}
}

@article{chernozhukov2018double,
  title={Double/debiased machine learning for treatment and structural parameters},
  author={Chernozhukov, Victor and Chetverikov, Denis and Demirer, Mert and Duflo, Esther and Hansen, Christian and Newey, Whitney and Robins, James},
  journal={The Econometrics Journal},
  volume={21},
  number={1},
  pages={C1--C68},
  year={2018},
  publisher={Oxford University Press Oxford, UK}
}

@article{wager2018estimation,
  title={Estimation and inference of heterogeneous treatment effects using random forests},
  author={Wager, Stefan and Athey, Susan},
  journal={Journal of the American Statistical Association},
  volume={113},
  number={523},
  pages={1228--1242},
  year={2018},
  publisher={Taylor \& Francis}
}

@Book{hernan2024,
    author    = "Hern{\'a}n, M. A. and Robins, J. M.",
    title     = "Causal Inference: What If",
    publisher = "Chapman \\& Hall/CRC",
    year      = 2024
}

@article{robins1994,
	title = {Estimation of {Regression} {Coefficients} {When} {Some} {Regressors} are not {Always} {Observed}},
	volume = {89},
	issn = {0162-1459, 1537-274X},
	url = {https://www.tandfonline.com/doi/full/10.1080/01621459.1994.10476818},
	doi = {10.1080/01621459.1994.10476818},
	language = {en},
	number = {427},
	urldate = {2024-03-10},
	journal = {Journal of the American Statistical Association},
	author = {Robins, J. M. and Rotnitzky, A. and Zhao, L.},
	month = sep,
	year = {1994},
	pages = {846--866},
}

@article{bang2005,
  title={Doubly robust estimation in missing data and causal inference models},
  author={Bang, H. and Robins, J. M.},
  journal={Biometrics},
  volume={61},
  number={4},
  pages={962--973},
  year={2005},
  publisher={Oxford University Press}
}



@article{athey2019,
   author = "Athey, Susan and Imbens, Guido W.",
   title = "Machine Learning Methods That Economists Should Know About", 
   journal= "Annual Review of Economics",
   year = "2019",
   volume = "11",
   number = "Volume 11, 2019",
   pages = "685-725",
   doi = "https://doi.org/10.1146/annurev-economics-080217-053433",
   url = "https://www.annualreviews.org/content/journals/10.1146/annurev-economics-080217-053433",
   publisher = "Annual Reviews",
   issn = "1941-1391",
   type = "Journal Article",
   keywords = "causal inference",
   keywords = "JEL C30",
   keywords = "machine learning",
   keywords = "econometrics",
   abstract = "We discuss the relevance of the recent machine learning (ML) literature for economics and econometrics. First we discuss the differences in goals, methods, and settings between the ML literature and the traditional econometrics and statistics literatures. Then we discuss some specific methods from the ML literature that we view as important for empirical researchers in economics. These include supervised learning methods for regression and classification, unsupervised learning methods, and matrix completion methods. Finally, we highlight newly developed methods at the intersection of ML and econometrics that typically perform better than either off-the-shelf ML or more traditional econometric methods when applied to particular classes of problems, including causal inference for average treatment effects, optimal policy estimation, and estimation of the counterfactual effect of price changes in consumer choice models.",
  }


@article{wager2018estimation,
  title={Estimation and inference of heterogeneous treatment effects using random forests},
  author={Wager, Stefan and Athey, Susan},
  journal={Journal of the American Statistical Association},
  volume={113},
  number={523},
  pages={1228--1242},
  year={2018},
  publisher={Taylor \& Francis}
}

@article{athey2016recursive,
  title={Recursive partitioning for heterogeneous causal effects},
  author={Athey, Susan and Imbens, Guido},
  journal={Proceedings of the National Academy of Sciences},
  volume={113},
  number={27},
  pages={7353--7360},
  year={2016},
  publisher={National Acad Sciences}
}

@article{shalit2017estimating,
  title={Estimating individual treatment effect: generalization bounds and algorithms},
  author={Shalit, Uri and Johansson, Fredrik D and Sontag, David},
  journal={International Conference on Machine Learning},
  pages={3076--3085},
  year={2017},
  organization={PMLR}
}

@inproceedings{louizos2017causal,
  title={Causal effect inference with deep latent-variable models},
  author={Louizos, Christos and Shalit, Uri and Mooij, Joris M and Sontag, David and Zemel, Richard and Welling, Max},
  booktitle={Advances in Neural Information Processing Systems},
  pages={6446--6456},
  year={2017}
}

@inproceedings{Ma2020CausalIU,
  title={Causal Inference under Networked Interference and Intervention Policy Enhancement},
  author={Yunpu Ma and Volker Tresp},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  year={2020},
  url={https://api.semanticscholar.org/CorpusID:233236161}
}

@article{tchetgen2020introduction,
  title={Introduction to proximal causal learning},
  author={Tchetgen Tchetgen, Eric J and Ying, Aolin and Cui, Yifan and Shi, Xu and Miao, Wang},
  journal={arXiv preprint arXiv:2009.10982},
  year={2020}
}

@inproceedings{saito2020counterfactual,
  title={Counterfactual Cross-Validation: Stable Model Selection Procedure for Causal Inference Models},
  author={Saito, Yuta and Yasui, Shota},
  booktitle={International Conference on Machine Learning},
  pages={8398--8407},
  year={2020},
  organization={PMLR}
}

@article{akiba2019optuna,
  title={Optuna: A next-generation hyperparameter optimization framework},
  author={Akiba, Takuya and Sano, Shotaro and Yanase, Toshihiko and Ohta, Takeru and Koyama, Masanori},
  journal={Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={2623--2631},
  year={2019}
}

@article{schuler2018comparison,
  title={A comparison of methods for model selection when estimating individual treatment effects},
  author={Schuler, Alejandro and Baiocchi, Michael and Tibshirani, Robert and Shah, Nigam},
  journal={arXiv preprint arXiv:1804.05146},
  year={2018}
}

@misc{loshchilov2019decoupledweightdecayregularization,
      title={Decoupled Weight Decay Regularization}, 
      author={Ilya Loshchilov and Frank Hutter},
      year={2019},
      eprint={1711.05101},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/1711.05101}, 
}

@inproceedings{
melnychuk2024bounds,
title={Bounds on Representation-Induced Confounding Bias for Treatment Effect Estimation},
author={Valentyn Melnychuk and Dennis Frauen and Stefan Feuerriegel},
booktitle={The Twelfth International Conference on Learning Representations},
year={2024},
url={https://openreview.net/forum?id=d3xKPQVjSc}
}

@inproceedings{
mahajan2024empirical,
title={Empirical Analysis of Model Selection for Heterogeneous Causal Effect Estimation},
author={Divyat Mahajan and Ioannis Mitliagkas and Brady Neal and Vasilis Syrgkanis},
booktitle={The Twelfth International Conference on Learning Representations},
year={2024},
url={https://openreview.net/forum?id=yuy6cGt3KL}
}

@article{Nie2017QuasioracleEO,
  title={Quasi-oracle estimation of heterogeneous treatment effects},
  author={Xinkun Nie and Stefan Wager},
  journal={Biometrika},
  year={2017},
  url={https://api.semanticscholar.org/CorpusID:85529052}
}

@article{lalonde1986evaluating,
  title={Evaluating the econometric evaluations of training programs with experimental data},
  author={LaLonde, Robert J},
  journal={The American Economic Review},
  pages={604--620},
  year={1986},
  publisher={JSTOR}
}

@article{neal2020realcause,
  title={RealCause: Realistic Causal Inference Benchmarking},
  author={Neal, Brady and Huang, Chin-Wei and Raghupathi, Sunand},
  journal={arXiv preprint arXiv:2011.15007},
  year={2020}
}

@article{dorie2019automated,
  title={Automated versus do-it-yourself methods for causal inference: Lessons learned from a data analysis competition},
  author={Dorie, Vincent and Hill, Jennifer and Shalit, Uri and Scott, Marc and Cervone, Dan},
  journal={Statistical Science},
  volume={34},
  number={1},
  pages={43--68},
  year={2019},
  publisher={Institute of Mathematical Statistics}
}


@InProceedings{pmlr-v162-melnychuk22a,
  title = 	 {Causal Transformer for Estimating Counterfactual Outcomes},
  author =       {Melnychuk, Valentyn and Frauen, Dennis and Feuerriegel, Stefan},
  booktitle = 	 {Proceedings of the 39th International Conference on Machine Learning},
  pages = 	 {15293--15329},
  year = 	 {2022},
  editor = 	 {Chaudhuri, Kamalika and Jegelka, Stefanie and Song, Le and Szepesvari, Csaba and Niu, Gang and Sabato, Sivan},
  volume = 	 {162},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {17--23 Jul},
  publisher =    {PMLR},
  pdf = 	 {https://proceedings.mlr.press/v162/melnychuk22a/melnychuk22a.pdf},
  url = 	 {https://proceedings.mlr.press/v162/melnychuk22a.html},
  abstract = 	 {Estimating counterfactual outcomes over time from observational data is relevant for many applications (e.g., personalized medicine). Yet, state-of-the-art methods build upon simple long short-term memory (LSTM) networks, thus rendering inferences for complex, long-range dependencies challenging. In this paper, we develop a novel Causal Transformer for estimating counterfactual outcomes over time. Our model is specifically designed to capture complex, long-range dependencies among time-varying confounders. For this, we combine three transformer subnetworks with separate inputs for time-varying covariates, previous treatments, and previous outcomes into a joint network with in-between cross-attentions. We further develop a custom, end-to-end training procedure for our Causal Transformer. Specifically, we propose a novel counterfactual domain confusion loss to address confounding bias: it aims to learn adversarial balanced representations, so that they are predictive of the next outcome but non-predictive of the current treatment assignment. We evaluate our Causal Transformer based on synthetic and real-world datasets, where it achieves superior performance over current baselines. To the best of our knowledge, this is the first work proposing transformer-based architecture for estimating counterfactual outcomes from longitudinal data.}
}


@article{
zhang2023exploring,
title={Exploring Transformer Backbones for Heterogeneous Treatment Effect Estimation},
author={YiFan Zhang and Hanlin Zhang and Zachary Chase Lipton and Li Erran Li and Eric Xing},
journal={Transactions on Machine Learning Research},
issn={2835-8856},
year={2023},
url={https://openreview.net/forum?id=1kl4YM2Q7P},
note={}
}

@article{zhang2023towards,
  title={Towards Causal Foundation Model: on Duality between Causal Inference and Attention},
  author={Zhang, Jiaqi and Jennings, Joel and Zhang, Cheng and Ma, Chao},
  journal={arXiv preprint arXiv:2310.00809},
  year={2023}
}

@article{Tchetgen2024,
author = {Eric J. Tchetgen Tchetgen and Andrew Ying and Yifan Cui and Xu Shi and Wang Miao},
title = {{An Introduction to Proximal Causal Inference}},
volume = {39},
journal = {Statistical Science},
number = {3},
publisher = {Institute of Mathematical Statistics},
pages = {375 -- 390},
keywords = {causality, confounding, counterfactual outcomes, negative control, proxies},
year = {2024},
doi = {10.1214/23-STS911},
URL = {https://doi.org/10.1214/23-STS911}
}

@inproceedings{
kompa2022deep,
title={Deep Learning Methods for Proximal Inference via Maximum Moment Restriction},
author={Benjamin Kompa and David Remy Bellamy and Tom Kolokotrones and James Robins and Andrew Beam},
booktitle={Advances in Neural Information Processing Systems},
editor={Alice H. Oh and Alekh Agarwal and Danielle Belgrave and Kyunghyun Cho},
year={2022},
url={https://openreview.net/forum?id=fRWwcgfXXZ}
}
